Tropical $k$-means clustering for phylogenetic trees

The asymmetric tropical distance is a distance measure on the tropical torus $\mathbb{R}^n/\mathbb{R}\mathbf{1}$ and in particular on the Bergman fan $B(K_N) \subseteq \mathbb{R}^{\binom{N}{2}}/\mathbb{R}\mathbf{1}$ of the complete graphical matroid. In this paper, we define and analyse a clustering algorithm for equidistant phylogenetic trees based on this distance, using the correspondence between $B(K_N)$ and the space of equidistant trees with $N$ leaves.

==> local_optimum.tikz.tex <==
\begin{tikzpicture}
  \coordinate (e1) at (2,0);                       % along x-axis
  \coordinate (e2) at ({2*cos(120)},{2*sin(120)});     % 120° from r
  \coordinate (e3) at ({3*cos(240)},{3*sin(240)});
  
  \draw (0,0) -- ($(e1)$);
  \draw (0,0) -- ($(e2)$);
  \draw (0,0) -- ($(e3)$);
\end{tikzpicture}
